Provably Efficient Reinforcement Learning for Online Adaptive Influence Maximization

Online influence maximization aims to maximize the influence spread of a content in a social network with unknown network model by selecting a few seed nodes. Recent studies followed a non-adaptive setting, where the seed nodes are selected before the start of the diffusion process and network parameters are updated when the diffusion stops. We consider an adaptive version of content-dependent online influence maximization problem where the seed nodes are sequentially activated based on real-time feedback. In this paper, we formulate the problem as an infinite-horizon discounted MDP under a linear diffusion process and present a model-based reinforcement learning solution. Our algorithm maintains a network model estimate and selects seed users adaptively, exploring the social network while improving the optimal policy optimistically. We establish $\widetilde O(\sqrt{T})$ regret bound for our algorithm. Empirical evaluations on synthetic network demonstrate the efficiency of our algorithm.

==> ack.tex <==
\begin{ack}
    Use unnumbered first level headings for the acknowledgments. All acknowledgments
    go at the end of the paper before the list of references. Moreover, you are required to declare
    funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
    More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2022/PaperInformation/FundingDisclosure}.
    
    
Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work might be exploited to propagate eval political ideas, fake news or rumors through the social networks.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See appendix}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See section of experiment and appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See figure \ref{fig-reward}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See appendix}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{We didn't use.}
  \item Did you mention the license of the assets?
    \answerNA{We didn't use.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{We didn't use.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We didn't use.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We didn't use.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> symbols.tex <==
\usepackage{enumitem}
\usepackage{comment} 
\usepackage{hyperref}
\usepackage{natbib}
\usepackage{bm}

\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{times}

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}


%------------ 
\newcommand{\edim}{\mathrm {dim_E}}
%------------


%--------------
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{result}{Result}
% \newtheorem{problem}{Problem}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{question}{Question}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{condition}[theorem]{Condition}
% \newtheorem{conjecture}[theorem]{Conjecture}

% \newtheorem{remark}{Remark}[section]
% \newtheorem{example}{Example}[section]






%simon's macro
%\newcommand{\RR}{\mathsf{R}}
\newcommand{\vct}{\boldsymbol }
%\newcommand{\mat}{\mathbf}
\newcommand{\rnd}{\mathsf}
\newcommand{\ud}{\mathrm d}
\newcommand{\nml}{\mathcal{N}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\hinge}{\mathcal{R}}
\newcommand{\kl}{\mathrm{KL}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\dir}{\mathrm{Dir}}
\newcommand{\mult}{\mathrm{Mult}}
\newcommand{\err}{\mathrm{err}}
%\newcommand{\sgn}{\mathrm{sgn}}
\renewcommand{\sp}{\mathrm{span}}
%\renewcommand{\span}{\mathrm{span}}
%\newcommand{\argmin}{\mathrm{argmin}}
%\newcommand{\argmax}{\mathrm{argmax}}
\newcommand{\poly}{\mathrm{poly}}
%\newcommand{\rank}{\mathrm{rank}}
%\newcommand{\conv}{\mathrm{conv}}
%\newcommand{\E}{\mathbb{E}}
%\newcommand{\diag}{\mathrm{diag}}
\newcommand{\acc}{\mathrm{acc}}
\newcommand{\ER}{\mathrm{ER}}

\newcommand{\aff}{\mathrm{aff}}
\newcommand{\range}{\mathrm{Range}}
\newcommand{\Sgn}{\mathrm{sign}}

\newcommand{\hit}{\mathrm{hit}}
\newcommand{\cross}{\mathrm{cross}}
\newcommand{\Left}{\mathrm{left}}
\newcommand{\Right}{\mathrm{right}}
\newcommand{\Mid}{\mathrm{mid}}
\newcommand{\bern}{\mathrm{Bernoulli}}
\newcommand{\ols}{\mathrm{ols}}
%\newcommand{\tr}{\mathrm{tr}}
\newcommand{\opt}{\mathrm{opt}}
%\newcommand{\ridge}{\mathrm{ridge}}
\newcommand{\unif}{\mathrm{unif}}
\newcommand{\Image}{\mathrm{im}}
\newcommand{\Kernel}{\mathrm{ker}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\pred}{\mathrm{pred}}
\newcommand{\distequal}{\stackrel{\mathbf{P}}{=}}
%\newcommand{\gege}{\textcircled{1}}
\newcommand{\gege}{{A(\vect{w},\vect{w}_*)}}
\newcommand{\gele}{{A(\vect{w},-\vect{w}_*)}}
\newcommand{\lele}{{A(-\vect{w},-\vect{w}_*)}}
\newcommand{\lege}{{A(-\vect{w},\vect{w}_*)}}
\newcommand{\firstlayer}{\mathbf{W}}
\newcommand{\firstlayerWN}{v}
\newcommand{\secondlayer}{a}
\newcommand{\inputvar}{\vect{x}}
\newcommand{\anglemat}{\mathbf{\Phi}}
\newcommand{\holder}{H\"{o}lder }
\newcommand{\real}{\mathbb{R}}
\newcommand{\approxerr}{\delta}

\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cK{\mathcal{K}}
\def\cS{\mathcal{S}}
\def\cI{\mathcal{I}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cW{\mathcal{W}}
\def\cZ{\mathcal{Z}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\SS{\mathbb{S}}
\def\NN{\mathbb{N}}
\def\bP{\mathbf{P}}
\def\TV{\mathrm{TV}}
\def\MSE{\mathrm{MSE}}
\def\intdim{\mathrm{intdim}}
\def\vw{\mathbf{w}}
\def\va{\mathbf{a}}
\def\vZ{\mathbf{Z}}

\newcommand{\mat}[1]{#1}
\newcommand{\vect}[1]{#1}
%%\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\normop}[1]{\left\|#1\right\|_{\mathrm{op}}}
\newcommand{\simplex}{\triangle}
%\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\prox}[2]{\textbf{Prox}_{#1}\left\{#2\right\}}
\newcommand{\event}[1]{\mathscr{#1}}
\newcommand{\set}[1]{#1}
\newcommand{\diff}{\text{d}}
%\newcommand{\train}{\text{tr}}
%\newcommand{\test}{\text{te}}
\newcommand{\apx}{\text{apx}}
\newcommand{\difference}{\triangle}
\newcommand{\inputdist}{\mathcal{X}}
\newcommand{\indict}{\mathbb{I}}
\newcommand{\rotmat}{\mathbf{R}}
\newcommand{\normalize}[1]{\overline{#1}}
\newcommand{\vectorize}[1]{\text{vec}\left(#1\right)}
\newcommand{\vclass}{\mathcal{G}}
\newcommand{\pclass}{\Pi}
\newcommand{\qclass}{\mathcal{Q}}
\newcommand{\rclass}{\mathcal{R}}
\newcommand{\classComplexity}[2]{N_{class}(#1,#2)}
\newcommand{\cclass}{\mathcal{F}}
\newcommand{\gclass}{\mathcal{G}}
\newcommand{\pthres}{p_{thres}}
\newcommand{\ethres}{\epsilon_{thres}}
\newcommand{\eclass}{\epsilon_{class}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\trans}{P}
\newcommand{\lowprobstate}{\psi}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\contexts}{\mathcal{X}}
\newcommand{\edges}{\mathcal{E}}
\newcommand{\variance}{\text{Var}}
\newcommand{\params}{\vect{w}}

\newcommand{\relu}[1]{\sigma\left(#1\right)}
\newcommand{\reluder}[1]{\sigma'\left(#1\right)}
\newcommand{\act}[1]{\sigma\left(#1\right)}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{asmp}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{oracle}{Oracle}[section]
%\newtheorem{fact}{Fact}[section]
\newtheorem{conj}{Conjecture}[section]
\newtheorem{rem}{Remark}[section]
%\newtheorem{example}{Example}[section]
%\newtheorem{condition}{Condition}[section]

%RL 
\newcommand{\levels}{[H]}
\newcommand{\fclass}{\mathcal{F}}
\newcommand{\covset}{\mathcal{M}}
\newcommand{\epsstat}{\epsilon_s}
\newcommand{\epstest}{\epsilon_t}
%\newcommand{\epsreg}{\epsilon_r}
\newcommand{\deltatrain}{\delta_{tr}}
\newcommand{\deltatest}{\delta_{te}}
\newcommand{\dist}{\mathcal{D}}
\newcommand{\gap}{\mathrm{gap}}
\newcommand{\gapmin}{\rho}
\newcommand{\algo}{\textsf{Difference Maximization $Q$-learning}}
\newcommand{\epsn}{\epsilon_N}
\newcommand{\ridge}{\lambda_{\mathrm{ridge}}}
\newcommand{\epsr}{\lambda_r}
\newcommand{\pifinal}{\hat{\pi}}
\newcommand{\true}{$\mathrm{True}$}
\newcommand{\false}{$\mathrm{False}$}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\relearn}{$NeedToReLearn$}
\newcommand{\distmdp}{\dist_{\mathrm{MDP}}}
\newcommand{\dmdp}{d_{\mathrm{MDP}}}
\newcommand{\linopt}{T}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\srl}{\textsf{RL}}
\newcommand{\gm}{\textsf{Generative Model}}
\newcommand{\kt}{\textsf{Known Transition}}
%\def\approxcorrect{\checkmark\kern-1.1ex\raisebox{.7ex}{\rotatebox[origin=c]{125}{--}}}
%\def\approxcorrect{\checkmark\kern-1.1ex\raisebox{.89ex}{$\xmark$}}
\def\approxcorrect{\cmark\kern-1.4ex\raisebox{.30ex}{$\xmark$}}
\newcommand{\spanner}{\Lambda}

\newcommand{\idx}{\textsf{INDEX-QUERY}}
\newcommand{\idxn}[1][]{\ifthenelse{\equal{#1}{}}{\mathbb{INDQ}_n}{\mathbb{INDQ}_{#1}}}
\newcommand{\reward}{\overline{r}}



%% TT's definitions
%\newcommand\tr{{{\operatorname{trace}}}}
%\newcommand{\eps}{\varepsilon}
%\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}

\newcommand{\el}{L}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
%\newcommand{\vc}[1]{{\text{vect}(#1)}}
\newcommand{\alpb}{\zeta}
\newcommand{\alpbb}{(\la -\eta\bp^2/2)\bn}
\newcommand{\gam}{{\gamma}}
\newcommand{\KB}{\bar{K}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
%\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\bp}{\beta}
\newcommand{\bn}{\alpha}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
%\newcommand{\vs}{{\vspace*{-4pt}}}
\newcommand{\eeq}{\end{equation}}
%\newcommand{\prox}{{{\text{\bf{prox}}}}}
%\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bt}{\bigotimes}
%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
%\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
%\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
%\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
%\newcommand{\diag}{\text{diag}}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Dc}{{\cal{D}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Vc}{{\cal{V}}}
%\newcommand{\Pb}{{\mtx{P}}}
%\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
%\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
% \newcommand{\Cb}{{\mtx{C}}}
% \newcommand{\Eb}{{\mtx{E}}}
% \newcommand{\Hb}{{\mtx{H}}}
% \newcommand{\Gc}{{\cal{G}}}
% \newcommand{\F}{{\mtx{F}}}
%\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
% \newcommand{\Db}{{\mtx{D}}}
% \newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\bx}{{\bm{x}}}
\newcommand{\bg}{{\bm{g}}}
\newcommand{\bw}{{\bm{w}}}
\newcommand{\br}{{\bm{r}}}
\newcommand{\ba}{{\bm{a}}}
\newcommand{\bu}{{\bm{u}}}
\newcommand{\bv}{{\bm{v}}}
\newcommand{\bz}{{\bm{z}}}
\newcommand{\be}{{\bm{e}}}
\newcommand{\by}{{\bm{y}}}
\newcommand{\bbw}{\bar{{\bm{w}}}}
\newcommand{\hbw}{\hat{{\bm{w}}}}
\newcommand{\hp}{\hat{p}}
\newcommand{\I}{{\text{I}}}
% \newcommand{\II}{{\text{II}}}
\newcommand{\btheta}{{\bm{\theta}}}
\newcommand{\bdelta}{{\bm{\delta}}}
%\newcommand{\balpha}{{\bm{\alpha}}}
\newcommand{\ulambda}{{\underline{\lambda}}}
\newcommand{\barlambda}{{\bar{\lambda}}}
\newcommand{\bphi}{{\bm{\phi}}}
\newcommand{\hphi}{{\hat{\phi}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
%\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\Otil}[1]{{\tilde{\cal{O}}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{\sigma_{\min}(#1)}}
\newcommand{\smx}[1]{{\sigma_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
% \newcommand{\zb}{{\bar{\z}}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tti}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
%\newcommand{\dist}[1]{\text{dist}(#1)}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Nc}{{\mathcal{N}}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bTeta}{\boldsymbol{\Theta}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathbb{S}^{n-1}}
\newcommand{\Mc}{\mathbb{S}^{dr-1}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
%\newcommand{\vb}{\vct{v}}
% \newcommand{\Jb}{\mtx{J}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
% \newcommand{\fb}{\vct{f}}
% \newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
%\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
% \newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\Wp}{\mtx{W}^\dagger}
% \newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
%\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
%\newcommand{\ab}{\vct{a}}
% \newcommand{\bb}{\vct{b}}
% \newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hW}{\hat{W}}
\newcommand{\hTheta}{\hat{\Theta}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}


%%YP's macros
%\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\qqq}[1]{{\textcolor{black}{{#1}}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
%\newcommand{\mat}[1]{{\text{mat}\left(#1\right)}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
%\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}
%\newcommand{\cF}{\mathcal{F}}
%\newcommand{\cH}{\mathcal{H}}
%\newcommand{\cA}{\mathcal{A}}
%\newcommand{\cD}{\mathcal{D}}
%\newcommand{\cX}{\mathcal{X}}
%\newcommand{\cN}{\mathcal{N}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
%\newcommand{\rb}{\vct{r}}
\newcommand{\rbt}{\vct{r}(\vct{\theta})}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
%\newcommand{\R}{\mathsf{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
%\newcommand{\Z}{\mathsf{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
%\newcommand{\Var}{\textrm{Var}}
%\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\renewcommand{\i}{\imath}

%\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

%\newcommand{\rank}{\operatorname{rank}}
%\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}
\newcommand{\cp}{R_{p}}
\newcommand{\cs}{\nu}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
%\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}



\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
%\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


%\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
%           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}

\newcommand{\shortrnote}[1]{ &  &  & \text{\footnotesize\llap{#1}}}
\newcommand{\longrnote}[1]{ &  &  \\   &  &  &  &  & \notag \text{\footnotesize\llap{#1}}}
\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\Trace}{{\mathrm{Tr}}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
%\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}


% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\minimize}{minimize}

%representation learning commands
\newcommand{\inputspace}{\cX}
\newcommand{\rep}{\phi}
\newcommand{\repclass}{\Phi}
\newcommand{\covdomc}{\mu}
\newcommand{\proj}{\mathrm{Proj}}
\newcommand{\divergence}{D}
\newcommand{\linlayer}{W}
\newcommand{\noise}{Z}
\newcommand{\noisebound}{b}
\newcommand{\error}{\epsilon}
\newcommand{\gausswidth}{\mathcal{G}}
\newcommand{\cover}{\mathcal{C}}
\newcommand{\diverge}{\mathsf{D}}
\newcommand{\thres}{\lambda}
\newcommand{\operator}{\mathbb{P}}

\newcommand{\normF}[1]{\|#1\|_F}
\newcommand{\normtwo}[1]{\|#1\|_2}

%author comments\
\newcommand{\kaixuan}[1]{\textcolor{purple}{[Kaixuan: #1]}}

